Partial Binarization of Neural Networks for Budget-Aware Efficient Learning

Binarization is a powerful compression technique for neural networks, significantly reducing FLOPs, but often results in a significant drop in model performance. To address this issue, partial binarization techniques have been developed, but a systematic approach to mixing binary and full-precision parameters in a single network is still lacking. In this paper, we propose a controlled approach to partial binarization, creating a budgeted binary neural network (B2NN) with our MixBin strategy. This method optimizes the mixing of binary and full-precision components, allowing for explicit selection of the fraction of the network to remain binary. Our experiments show that B2NNs created using MixBin outperform those from random or iterative searches and state-of-the-art layer selection methods by up to 3% on the ImageNet-1K dataset. We also show that B2NNs outperform the structured pruning baseline by approximately 23% at the extreme FLOP budget of 15%, and perform well in object tracking, with up to a 12.4% relative improvement over other baselines. Additionally, we demonstrate that B2NNs developed by MixBin can be transferred across datasets, with some cases showing improved performance over directly applying MixBin on the downstream data.

==> plot_tex/choice_of_activation.tex <==
\begin{wrapfigure}{R}{6cm}
%\begin{figure}[ht]
\centering
  \includegraphics[width=1\linewidth]{figures/fig_choice_of_activation.pdf}
  \caption{\udbhb{TODO: shift this figure to left} Performance of B2NN with different activation functions. Here, B2NNs are constructed by random selection. CIFAR-ResNet20, CIFAR100}
    \label{fig-activations-out}
%\end{figure}
\end{wrapfigure}




==> plot_tex/different_activations.tex <==
% \begin{wrapfigure}{R}{7cm}
% %\begin{figure}[ht]
% \vspace{-1em}
% \centering
%   \includegraphics[width=\linewidth]{iclr2022/figures/fig_different_activation_functions.pdf}
%   \caption{Schematic representation of BinReLU and other activation functions for an input range of [-2, 2].}
%     \label{fig-activations}
% \vspace{-2em}
% \end{wrapfigure}
%\end{figure}

\begin{figure}
\centering
  \includegraphics[width=0.8\linewidth]{figures/fig_different_activation_functions.pdf}
  \caption{Schematic representation of BinReLU and other activation functions for an input range of [-2, 2].}
  \label{fig-activations}
  \end{figure}
\begin{figure}
\centering
  \includegraphics[width=0.7\linewidth]{figures/fig_choice_of_activation.pdf}
  \caption{Performance of B2NNs with different activation functions obtained at various FLOPs on CIFAR100 with cResNet20 model.}   
  \label{fig-activations-out}
\end{figure}

The proposed BinReLU activation function is designed to enhance the stability of the full-precision as well as binary components of a B2NN in general. Mathematically, BinReLU can be stated as 
\begin{equation}
    f(x) = 
    \begin{cases}
    -1 \text{ if } x \leq -1 \\
    x \text{ otherwise}
    \end{cases},
\end{equation}
where $x$ and $f(x)$ denote the input and output of the activation function. 

Figure \ref{fig-activations} shows the BinReLU function together with ReLU, HardTanh and Identify mappings. For full-precision networks, ReLU is considered a very effective choice of activation, however, since it eliminates the activation information below 0, it does not work well for binary networks. For BNNs, either of HardTanh or Identity functions are preferred. However, both these activations do not work well for the real-valued networks (Figure \ref{fig-activations-out}). Note that an identity mapping works well for BNN since for such cases, nonlinearity is inherently introduced through the squashing of the activation values to -1 and 1 using Sign$(\cdot)$ as denoted in Eq. \ref{eq-sign}. BinReLU is inspired from the other activations stated here in a sense that it preserves the characteristics of ReLU for positive activations and keeps them real-valued, and also ensures that the activation information between -1 and 0 is preserved.


==> plot_tex/effect_of_random_seed.tex <==
% \begin{minipage}{0.32\textwidth}
\begin{figure}\centering
\centering
\includegraphics[width=0.7\linewidth]{figures/fig_effect_of_random_seed.pdf}
\caption{Performance scores obtained with different random seeds for with \texttt{MixBin} for the various compression levels of cResnet20 on CIFAR100 dataset.}
\label{fig-random}
\end{figure}

  



==> plot_tex/object_detector.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{figures/fig_ObjTracker.pdf}
\caption{Performance of SiamFC and its different compressed variants obtained using B2NNs with different combinations of full-precision and binary layers. }
\label{fig-tracking}
\end{figure}



